Non-Sequential Graph Script Induction via Multimedia Grounding

Online resources such as WikiHow compile a wide range of scripts for performing everyday tasks, which can assist models in learning to reason about procedures. However, the scripts are always presented in a linear manner, which does not reflect the flexibility displayed by people executing tasks in real life. For example, in the CrossTask Dataset, 64.5% of consecutive step pairs are also observed in the reverse order, suggesting their ordering is not fixed. In addition, each step has an average of 2.56 frequent next steps, demonstrating "branching". In this paper, we propose the new challenging task of non-sequential graph script induction, aiming to capture optional and interchangeable steps in procedural planning. To automate the induction of such graph scripts for given tasks, we propose to take advantage of loosely aligned videos of people performing the tasks. In particular, we design a multimodal framework to ground procedural videos to WikiHow textual steps and thus transform each video into an observed step path on the latent ground truth graph script. This key transformation enables us to train a script knowledge model capable of both generating explicit graph scripts for learnt tasks and predicting future steps given a partial step sequence. Our best model outperforms the strongest pure text/vision baselines by 17.52% absolute gains on F1@3 for next step prediction and 13.8% absolute gains on Acc@1 for partial sequence completion. Human evaluation shows our model outperforming the WikiHow linear baseline by 48.76% absolute gains in capturing sequential and non-sequential step relationships.

==> cache/2_motivation.tex <==

\section{Motivation}

\subsection{From instructional text/video to Multimedia Schema}


Existing online instructional text as shown in Fig.\ref{fig:schema} always consist of a sequential ordering of steps. This sequential ordering is useful in introducing one possible path towards completing the given task. However, such an over-simplified linear step sequence only offers a small glimpse into the whole picture of the task. As shown in Fig.\ref{fig:schema}, most everyday tasks are not as simple as following a ordered set of steps. Tasks usually consist of interchangeable steps that can occur in any order and optional steps that may or may not be performed based on user preference. Only learning from such existing one-dimensional instructions will limit users' understanding of the various possible paths that lead to successful completion of the task and hinder their ability to choose the best applicable path for their unique circumstance.


To address this over-simplification weakness of existing online instructional text, we propose to generate non-sequential multimedia task schemata that are able to capture interchangeable and optional orderings of steps as shown in Fig.\ref{fig:schema}. Ideally, such schemata should present users with a complete perspective on completing the task that include multiple valid paths all leading to successful task completion.



\subsection{Benefits from video data}

Textual scripts are prone to reporting bias: some events and information are omitted since the author considers them to be commonsense. In this case, video data can provide additional details to each step that textual descriptions do not explicitly mention.

Text scripts are usually more rigid / static compared to videos. Such online instructional text for given tasks often adhere to similar methodologies with very limited variations. Using video data helps to alleviate this problem by introducing many creative methodologies from online content creators that may not be as widely recognized/adopted but works just as well.

\subsection{Benefits from textual data}

Video data usually comes with high background variance and noise. It is difficult for the model to differentiate between essential task-related information and non-essential noise. For example in the aforementioned cooking scenario, the background kitchen environment and unique set of cooking utensils used by different chefs do not contribute useful information to our schema, yet they take up large portions of the video frames.

Grounding these video frames to a consistent textual step library can solve this generalization problem. In this process, non-essential background information is filtered out and essential task-related information is preserved.



\begin{figure*}[ht]
\begin{center}
\includegraphics[width=80mm,scale=0.5]{image/contrast.png}
\end{center}
\caption{Online sequential instructional video and text in contrast to our Multimedia Schema}
\label{fig:schema}
\end{figure*}

==> init.tex <==
\pdfoutput=1

\usepackage[table,dvipsnames]{xcolor}
\usepackage{times}
\usepackage{latexsym}
% \renewcommand{\UrlFont}{\ttfamily\small}

% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
\usepackage[T1]{fontenc}
% For Vietnamese characters
% \usepackage[T5]{fontenc}
% See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

\usepackage[dvipsnames]{xcolor}


% This assumes your files are encoded as UTF8
\usepackage[utf8]{inputenc}

% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
\usepackage{microtype}
\usepackage{hyperref}
% If the title and author information does not fit in the area allocated, uncomment the following
%
%\setlength\titlebox{<dim>}
%
% and set <dim> to something 5cm or larger.



%\setlength\titlebox{5cm}
% You can expand the titlebox if you need extra space
% to show all the authors. Please do not make the titlebox
% smaller than 5cm (the original size); we will check this
% in the camera-ready version and ask you to change it back.

\renewcommand*{\ttdefault}{cmtt}
\usepackage{graphicx}               % Include graph
\usepackage{tabularx}               % Better table formatting
\newcolumntype{C}{>{\centering\arraybackslash}X}
\usepackage{multirow}               % Multi-row in tables
\usepackage{diagbox}                % Diagonal line in tables
\usepackage{hhline}                 % Draw double line in tables
\usepackage{color}                  % Text and background color
\usepackage{amsmath}                % Formula
\usepackage{amssymb}                % Formula
\usepackage{mathtools}              % Formula
\usepackage{enumitem}               % Better itemize environment
\usepackage[ruled,vlined]{algorithm2e}

\newcommand{\bs}{\boldsymbol}
\newcommand{\mr}{\mathrm}
\newcommand{\ola}{\overleftarrow}
\newcommand{\ora}{\overrightarrow}
\newcommand{\real}{\mathbb{R}}
\newcommand{\ccgreen}{\cellcolor{Emerald!10}}
\newcommand{\ccdgreen}{\cellcolor{Emerald!20}}
\newcommand{\ccddgreen}{\cellcolor{Emerald!35}}
\newcommand{\x}{\checkmark}
%\usepackage{caption}
\usepackage{subcaption}
\usepackage{booktabs}
\usepackage{extarrows}
\usepackage{makecell}
\usepackage{dutchcal}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}  

\newtheorem{thm:def}{Definition}
\newtheorem{thm:eg}{Example}
\newtheorem{thm:lem}{Lemma}

\newcommand{\instancegraph}{g} % g^\mathbb{I}
\newcommand{\schemagraph}{s} % g^\mathbb{S}
\newcommand{\instancegraphset}{\mathcal{G}} % G^\mathbb{I}
\newcommand{\schemagraphset}{\mathcal{S}} % G\textsuperscript{$\mathbb{S}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}


\definecolor{RoseQuartzBg}{HTML}{F7CAC9}
\definecolor{RoseQuartz}{HTML}{F5A798}
\definecolor{Serenity}{HTML}{92A8D1}
\definecolor{OrangeRed}{rgb}{1.0, 0.27, 0.0}
\definecolor{Turquoise}{HTML}{0F4C81}
\definecolor{mint}{rgb}{0.24, 0.71, 0.54}


\usepackage{xparse}
\NewDocumentCommand{\heng}
{ mO{} }{\textcolor{OrangeRed}{\textsuperscript{\textit{Heng}}\textsf{\textbf{\small[#1]}}}}
\NewDocumentCommand{\revanth}
{ mO{} }{\textcolor{Cyan}{\textsuperscript{\textit{Revanth}}\textsf{\textbf{\small[#1]}}}}
% \NewDocumentCommand{\manling}{ mO{} }{\textcolor{Cyan}{\textsuperscript{\textit{Manling}}\textsf{\textbf{\small[#1]}}}}
\NewDocumentCommand{\manling}{ mO{} }{#1}


\newcommand\topalign[1]{%
  \setbox0\hbox{#1}%
  \raisebox{\dimexpr-\ht0+\dp0\relax}{\usebox0}}






